Unauthorized Drone Detection: Experiments and Prototypes

The increase in the number of unmanned aerial vehicles a.k.a. drones pose several threats to public privacy, critical infrastructure and cyber security. Hence, detecting unauthorized drones is a significant problem which received attention in the last few years. In this paper, we present our experimental work on three drone detection methods (i.e., acoustic detection, radio frequency (RF) detection, and visual detection) to evaluate their efficacy in both indoor and outdoor environments. Owing to the limitations of these schemes, we present a novel encryption-based drone detection scheme that uses a two-stage verification of the drone's received signal strength indicator (RSSI) and the encryption key generated from the drone's position coordinates to reliably detect an unauthorized drone in the presence of authorized drones.

==> figures/fig_rf_results1.tex <==


\begin{figure}[!h]
\centering
\subcaptionbox{Frequency content of the received signal with (top) and without (bottom) controller signal (Performed in QMIC's office corridors).}{\includegraphics[width=6cm, height=3cm]{figures/rf-qmic.png}}%rf-roc.png
\vspace{2em}
\subcaptionbox{Frequency content of the received signal with (top) and without (bottom) controller signal (Performed in Parking Area).}{\includegraphics[width=6cm, height=3cm]{figures/rf-parking.png}}%rf-precision.png
\caption{RF-based detection: Analysis of received signal.}
\label{fig_rf_results1}
\end{figure}

==> figures/fig_visual_proto.tex <==

\begin{figure}[!h]
\centering

%%% ======= Method 1
% \subcaptionbox{\scriptsize Web interface showing system parameters.}{\includegraphics[width=0.8\columnwidth]{figures/camera1.jpg}}%
% \vspace{2em}
% \subcaptionbox{\scriptsize Web interface showing camera FOV in real time.}{\includegraphics[width=0.8\columnwidth]{figures/camera2.jpg}}%

%%% ======= Method 2
% \begin{adjustbox}{minipage=0.8\columnwidth, precode=\dbox}
\centering
% \subfloat[Web interface showing system parameters.]{\frame{\includegraphics[width=0.9\columnwidth, frame=3pt]{figures/camera1.jpg}}} \\[2em]
% \subfloat[Web interface showing camera FOV in real time.]{\includegraphics[width=0.9\columnwidth, frame=3pt]{figures/camera2.jpg}}
% \end{adjustbox}
\includegraphics[width=0.9\columnwidth, frame=3pt]{figures/camera2.jpg}
\caption{Graphical interface of camera-based detection prototype system showing drone (red circle) and camera's FOV (green beam).}
\label{fig_visual_proto}
\end{figure}
